Robust Dynamic Staffing with Predictions

We consider a natural dynamic staffing problem in which a decision-maker sequentially hires workers over a finite horizon to meet an unknown demand revealed at the end. Predictions about demand arrive over time and become increasingly accurate, while worker availability decreases. This creates a fundamental trade-off between hiring early to avoid understaffing (when workers are more available but forecasts are less reliable) and hiring late to avoid overstaffing (when forecasts are more accurate but availability is lower). This problem is motivated by last-mile delivery operations, where companies such as Amazon rely on gig-economy workers whose availability declines closer to the operating day. To address practical limitations of Bayesian models (in particular, to remain agnostic to the underlying forecasting method), we study this problem under adversarial predictions. In this model, sequential predictions are adversarially chosen uncertainty intervals that (approximately) contain the true demand. The objective is to minimize worst-case staffing imbalance cost. Our main result is a simple and computationally efficient online algorithm that is minimax optimal. We first characterize the minimax cost against a restricted adversary via a polynomial-size linear program, then show how to emulate this solution in the general case. While our base model focuses on a single demand, we extend the framework to multiple demands (with egalitarian/utilitarian objectives), to settings with costly reversals of hiring decisions, and to inconsistent prediction intervals. We also introduce a practical "re-solving" variant of our algorithm, which we prove is also minimax optimal. Finally we conduct numerical experiments showing that our algorithms outperform Bayesian heuristics in both cost and speed, and are competitive with (approximate or exact) Bayesian-optimal policies when those can be computed.

==> New_Results/imperfect-prediction.tex <==
\label{sec:imperfect prediction}


In this section, we consider relax the consistency of predictions (Assumption~\ref{asp:prediction sequence}) with the following relaxed version:

\begin{assumption}
\label{asp:prediction sequence epsilon relaxation}
    For all day $t\in[T]$, prediction $\predictiont$ satisfies 
    \begin{enumerate}
        \item \underline{{Bounded bias}}: 
        there exists $\biaseddemand_t$ such that $\abs{\demand - \biaseddemand_t}\leq \predictionbias_t$ and $\biaseddemand_t \in [\pLt,\pRt]$. Here $\{\predictionbias_t\}_{t\in[T]}$ is called the ``prediction bias upper bounds'', and is known to the platform.
        \item \underline{{Bounded variance}}: the prediction error is bounded, i.e., $\pRt - \pLt \leq \perrort$ for $\perrort>0$. Here $\{\perrort\}_{t\in[T]}$ is called ``prediction variance upper bounds'', and is known to the platform.
    \end{enumerate}
\end{assumption}
One interpretation of \Cref{asp:prediction sequence epsilon relaxation} is follows: the unknown demand $\demand$ on the operating day $T + 1$ might change over the hiring horizon ($t = 1, \dots, T$), which we denote by $\{\biaseddemand_t\}_{t\in[T]}$. These changes might be due to some external shocks (e.g., an unexpected high-volume traffic that boosts the transaction in Amazon) or internal managerial changes (e.g., misalignment between inventory management and sale) that cannot be captured in the predictions (generated from machine learning models). Such changes can also be viewed as the bias of the machine learning models that generate predictions.
The original Assumption~\ref{asp:prediction sequence} is a special case of Assumption~\ref{asp:prediction sequence epsilon relaxation} with prediction bias $\predictionbias_t = 0$ for all $t\in[T]$. Without the consistency property in Assumption~\ref{asp:prediction sequence}, in this section we do not assume that all prediction intervals are nested, nor $\{\perror_t\}_{t\in[T]}$ is decreasing in $t$. For our later analysis, we also introduce dummy notations $\predictionbias_0 = 0$ and $\perror_0 = \pRzero - \pLzero$.

\xhdr{The minimax optimal algorithm and analysis.}
Following the recipe of \Cref{sec:base model}, we introduce the following new linear program, with variables $\{\allocit,\lgap,\rgap\}_{i\in[n],t\in[T]}$, that characterizes the optimal minimax cost:
\begin{align}
\tag{$\textsc{LP-BiasVar}$}
    \label{eq:opt reduced form imperfect prediction}
    &\arraycolsep=1.4pt\def\arraystretch{2.2}
    \begin{array}{llll}
    \min\limits_{\substack{\xbf,\lgap,\rgap\geq \zerobf}}
    \qquad
    &
    \undercost\cdot \rgap\vee
    \overcost\cdot \lgap
    & 
    \text{s.t.}
    \\
    &
    \displaystyle\sum\nolimits_{t\in[T]}\frac{1}{\wdiscountit}\allocit \leq \supplyi
    &
    i\in[n]
    \\
    &
    \displaystyle\sum\nolimits_{i\in[n]}
    % \left(
    \sum\nolimits_{t\in[T]}
    \priceit \cdot \allocit 
    % +
    % \sum\nolimits_{t\in[k+1:T]}
    % \priceit \cdot \hallocijtk
    % \right)
    \leq \budget
    \quad
    &
    % k\in[0:T]
    \\
    &
    \displaystyle\sum\nolimits_{i\in[n]}\sum\nolimits_{t\in[k]}
    \allocit \leq 
    \max_{k'\in[0:k]}\plus{\pRzero - \perror_{k'} - 2\predictionbias_{k'}} + \lgap
    \quad\quad
    &
    k\in[T]
    \\
    &
    \displaystyle\sum\nolimits_{i\in[n]}\sum\nolimits_{t\in[T]}
    \allocit \geq \pRzero - \rgap
    &
\end{array}
\end{align}
% \vm{there is an $l$ in the middle of the program; seems a typo?}
% \yfcomment{fixed}

Program~\ref{eq:opt reduced form imperfect prediction} is a natural generalization of program~\ref{eq:opt reduced form} in \Cref{sec:base model} when we relax the consistency property of predictions and consequently the assumption that $\perrort$ is decreasing in $t$. Following the same intuition behind~\ref{eq:opt reduced form}, ~\ref{eq:opt reduced form imperfect prediction} essentially characterizes the cost guarantee and the canonical staffing profile of online algorithms that are candidates for optimality against a particular subset of adversarial prediction sequences (see eqn.\ \eqref{eq:single switch prediction construction imperfect prediction} in \Cref{apx:optalgimperfect}). 






Now we present the minimax optimal algorithm under Assumption~\ref{asp:prediction sequence epsilon relaxation} and its guarantee of optimality  (\Cref{thm:opt alg imperfect prediction}). It is worthwhile highlighting that Procedure~\ref{alg:emulator} is invoked as a subroutine with constructed prediction sequence $\{[\tilde\pL_t, \tilde\pR_t]\}_{t\in[T]}$ that satisfies the nested structure and decreasing width, i.e., $\tilde\pR_t - \tilde\pL_t$. This enables us to use \Cref{lem:emulator} of Procedure~\Cref{alg:emulator} for proving \Cref{thm:opt alg imperfect prediction}. The formal proof of \Cref{thm:opt alg imperfect prediction} is deferred to \Cref{apx:optalgimperfect}.

\begin{algorithm}
    \SetKwInOut{Input}{input}
    \SetKwInOut{Output}{output}
    \Input{prediction sequence $\predictions=\{[\pLt,\pRt]\}_{t\in[T]}$ revealed sequentially over time}
    \Output{staffing profile $\xbf$}
    \vspace{2mm}
    find an optimal solution $(\xbf^*, \lgap^*, \rgap^*)$ of program~\ref{eq:opt reduced form imperfect prediction}
    
    \vspace{2mm}
    invoke Procedure~\ref{alg:emulator} with canonical staffing profile $\canxbf \gets \xbf^*$ and prediction sequence $\tilde\predictions$ where $\tilde\pRt \gets \min_{\tau\in[0:t]} \pR_{\tau} + \predictionbias_{\tau}$, $\tilde\pLt \gets \max_{\tau\in[0:t]}\plus{\pL_{\tau} - \predictionbias_{\tau}}$ for every $t\in[T]$
    \caption{\OPTSimImperfect}
    \label{alg:opt imperfect prediction}
\end{algorithm}

\begin{restatable}{theorem}{optalgimperfect}
\label{thm:opt alg imperfect prediction}
    Under Assumption~\ref{asp:prediction sequence epsilon relaxation},
    \OPTSimImperfect\ is minimax optimal. Its optimal minimax cost $\optcost$ is equal to the objective value of~\ref{eq:opt reduced form imperfect prediction}.
\end{restatable}



==> New_Results/numerical.tex <==
In this section, we provide numerical justifications for the performance of our algorithm on synthetic instances.

\newcommand{\dailydemand}{\delta}
\newcommand{\dailydemands}{\boldsymbol{\dailydemand}}
\newcommand{\dailydemandt}{\dailydemand_t}
\newcommand{\prior}{\xi}
\newcommand{\priors}{\boldsymbol{\prior}}
\newcommand{\priort}{\prior_t}
\newcommand{\priork}{\prior_k}

\newcommand{\dailydemandsample}{\tilde{\dailydemand}}
\newcommand{\dailydemandsamples}{\tilde{\dailydemands}}
\newcommand{\dailydemandsamplest}{\dailydemandsamples\ted}
\newcommand{\dailydemandsamplesk}{\dailydemandsamples\ked}
\newcommand{\dailydemandsampletk}{\dailydemandsample\ted_k}
\newcommand{\dailydemandsamplekt}{\dailydemandsample\ked_t}

\newcommand{\estimateddemand}{\tilde{\demand}}
\newcommand{\estimateddemandk}{\estimateddemand\ked}

\xhdr{Experimental setup.} We generate the following staffing instances. There is a single delivery station with unknown demand $\demand$ on operating day $T + 1 \triangleq 15$. There are two workforce supply pools, each with $\supplyi \triangleq 30$ workers initially. We refer to the first workforce pool and the second workforce pool as ``fixed workers'' and ``ready workers'', respectively. The fixed workers need to be hired ten days before the operating day, i.e., $\wdiscount_{1t}\triangleq \indicator{t \leq 4}$ for every $t\in[14]$. Meanwhile, the ready workers have a s-shaped availability rate defined as $\wdiscount_{2t} \triangleq \frac{1}{1 + \exp(t - 9)}$ for every $t\in[14]$. Finally, there is an infinite budget for the platform.

We next describe the stochastic process generating demand $\demand$ and prediction sequences~$\predictions$. The total demand $\demand$ can be divided into $\dailydemands = \{\dailydemandt\}_{t\in[T]}$ such that $\sum_{t\in[T]}\dailydemandt = \demand$. Here $\dailydemandt$ is the partial demand that the platform observes in each day $t\in[T]$. In particular, each partial demand $\dailydemandt$ is realized from binomial distribution $\texttt{binom}(5, \priort)$ independently, where success probability (aka., prior) $\priort$ is itself realized from uniform distribution $\texttt{U}(0, 1)$ independently. The platform does not observe $\{\priort\}_{t\in[T]}$ through the entire workforce planning horizon, and only observes partial demand $\dailydemandt$ at the beginning of each day $t\in[T]$. In addition, the platform has access to machine learning technology. Specifically, in each day $k\in[T]$, the platform also receives a sampled partial demand profile $\dailydemandsamplesk = \{\dailydemandsamplekt\}_{t\in[T]}$ where $\dailydemandsamplekt$ is realized  from binomial distribution $\texttt{binom}(5, \priort)$ independently, i.e., sampled partial demand $\dailydemandsamplekt$ and partial demand $\dailydemandt$ are i.i.d.\ generated. \yfcomment{We can incorporate bias into our experiment by assuming $\dailydemandsamplekt$ is realized from $\texttt{binom}(5, \priort + \epsilon\ked_t)$.} 

The platform constructs prediction intervals $\predictions=\{[\pLt,\pRt]\}_{t\in[T]}$ using the observed partial demands and sampled partial demand profiles. Specifically, for each day $k\in[T]$, given observed partial demands $\{\dailydemandt\}_{t\in[k]}$ and sampled partial demand profiles $\{\dailydemandsamplest\}_{t\in[k]}$ in the first $k$ days, the platform computes a point estimator $\estimateddemandk$ as 
\begin{align}
\label{eq:numerical point estimator}
    \estimateddemandk \triangleq \sum_{t\in[k]}\dailydemandt + \frac{1}{k}\sum_{\tau\in[k]}\sum_{t\in[k+1:T]}\dailydemandsample^{(\tau)}_t
\end{align}
As a sanity check, given any prior profile $\priors=\{\priort\}_{t\in[T]}$, unknown demand $\demand$ and point estimator $\estimateddemandk$ have the same expectation, i.e., $\expect{\demand\condition \priors} = \expect{\estimateddemandk\condition\priors}$ for every $k\in[T]$. Given point estimator $\estimateddemandk$ for day $k$, the platform constructs the prediction interval $[\pL_k,\pR_k]$ as
\begin{align}
\label{eq:numerical prediction interval}
    \pL_k \triangleq \estimateddemandk - l_k \;\;\mbox{and}\;\; \pR_k \triangleq \estimateddemandk + r_k
\end{align} 
Here, $l_k$ and $r_k$ are constant such that
\begin{align*}
    \prob{\sum_{t\in[k+1:T]}\dailydemandt \geq \frac{1}{k}\sum_{\tau\in[k]}\sum_{t\in[k+1:T]}\dailydemandsample^{(\tau)}_t - l_k} =
    \prob{\sum_{t\in[k+1:T]}\dailydemandt \leq \frac{1}{k}\sum_{\tau\in[k]}\sum_{t\in[k+1:T]}\dailydemandsample^{(\tau)}_t + r_k} = 90\%
\end{align*}
where the randomness is take over prior profile $\priors$, partial demand profile $\dailydemands$, and sampled partial demand profiles $\{\dailydemandsamplest\}_{t\in[k]}$.

We formalize the timeline of the demand and prediction sequence generating process below.
\begin{itemize}
    \item On day 0: prior profile $\priors = \{\priort\}_{t\in[T]}$ are realized i.i.d.\ from uniform distribution $\texttt{U}(0, 1)$. Prior profile $\priors$ remains unknown to the platform through the whole decision horizon.
    \item On each day $t\in[T]$:
    \begin{itemize}
        \item partial demand $\dailydemandt$ is revealed to the platform from binomial distribution $\texttt{binom}(5, \priort)$,
        \item sample partial demand profile $\dailydemandsamplest = \{\dailydemandsampletk\}_{k\in[T]}$ where $\dailydemandsampletk$ is realized  from binomial distribution $\texttt{binom}(5, \priork)$ independently
        \item point estimator $\estimateddemandk$ defined in eqn.~\eqref{eq:numerical point estimator} and prediction interval $[\pL_k,\pR_k]$ defined in eqn.~\eqref{eq:numerical prediction interval} are constructed correspondingly.
    \end{itemize}
\end{itemize}

\xhdr{Policies.} In our numerical experiments, we compare the staffing cost of six different policies:
\begin{enumerate}
    \item FMNN: the minimax optimal algorithm (\Cref{alg:opt}).
    \item FMNN*: the minimax optimal algorithm that resolves \ref{eq:opt reduced form} in each day.
    \item A-GR: for each day $t\in[T]$, compute $\hat\demand_t \triangleq \frac{\overcost\pLt + \undercost\pRt}{\overcost+\undercost}$, and hire as much as possible in the current day $t$ to meet $\hat{d}_t$. 
    \item P-GR: for each day $t\in[T]$, compute $\hat\demand_t \triangleq \frac{\overcost\pLt + \undercost\pRt}{\overcost+\undercost}$ is the final demand, and hire as less as possible in the current day $t$ so that $\hat{d}_t$ can still be achieved in day $t + 1$.
    \item A-SIM: for each day $k\in[T]$, solve $\hat\demand_k$ as the optimal solution of the single-shot newsvendor problem where the demand distribution is the empirical distribution over samples $\{\sum_{t\in[k]}\dailydemandt + \sum_{t\in[k+1:T]}\dailydemandsample^{(\tau)}_t\}_{\tau\in[k]}$. Hire as much as possible in the current day $k$ to meet $\hat{d}_k$. 
    \item P-SIM: for each day $k\in[T]$, solve $\hat\demand_k$ as the optimal solution of the single-shot newsvendor problem where the demand distribution is the empirical distribution over samples $\{\sum_{t\in[k]}\dailydemandt + \sum_{t\in[k+1:T]}\dailydemandsample^{(\tau)}_t\}_{\tau\in[k]}$. hire as less as possible in the current day $k$ so that $\hat{d}_k$ can still be achieved in day $k + 1$. 
\end{enumerate}

\xhdr{Results.} We numerical evaluate the performances of all policies using Monte-Carlo simulation. For each parameter setup, we conduct 100 iterations of the simulation and records the empirical performance of each policy. In \Cref{fig:numerical result symmetric cost,fig:numerical result large under cost,fig:numerical result large over cost}, we plots three scenarios: symmetric overstaffing and understaffing cost ($\overcost = \undercost=1$), significantly larger understaffing cost ($\overcost = 1,\undercost = 10$), and significantly larger overstaffing cost ($\overcost = 10,\undercost = 1$). In all three scenarios, FMNN and FMNN* are weakly better than other four heuristics, A-GR, P-GR, A-SIM, P-SIM in both empirical median and empirical mean.

\begin{figure}
    \centering
    \includegraphics[scale = 0.5]{New Results/figs/symmetric-cost.png}
    \caption{Symmetric overstaffing and understaffing cost, $\overcost = \undercost = 1$.}
    \label{fig:numerical result symmetric cost}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[scale = 0.5]{New Results/figs/asymmetric-cost.png}
    \caption{Asymmetric overstaffing and understaffing cost, $\overcost = 1, \undercost = 10$.}
    \label{fig:numerical result large under cost}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[scale = 0.5]{New Results/figs/asymmetric-cost-2.png}
    \caption{Asymmetric overstaffing and understaffing cost, $\overcost = 10, \undercost = 1$.}
    \label{fig:numerical result large over cost}
\end{figure}

\newpage

==> Paper/EC-apx-related.tex <==
\section{Further Related Work}
\label{sec:further}
\input{Paper/related-work}

==> Paper/EC-extension.tex <==
\label{sec:extension}
In this section, we discuss generalizing our approach in \Cref{sec:base model} to two practically relevant extensions. To simplify the presentation, we impose perfect consistency (i.e., $\pbiass = \zerobf$) on the prediction intervals and assume them to be nested throughout this section. All our results can be extended under $\pbiass$-consistency in a straightforward fashion.

\vspace{-1mm}
\subsection{Workforce Planning for Multiple Stations}
\label{sec:multiple-station}
In last-mile delivery, which is the primary motivating application in our paper, the platform might prefer to couple the staffing decisions for various stations that share the same pools of workers (say, due to their geographical proximity), but have different unknown demands and heterogeneous prediction sequences. We start by generalizing our model to capture this extension and then study extending our algorithmic approach to two objective functions applicable in this new model, namely \emph{egalitarian}  and \emph{utilitarian} staffing cost functions. 

\xhdr{The multi-station environment.} We consider the setting in which the platform manages staffing decisions for $m$ delivery stations. Each delivery station $j\in[m]$ has an unknown target staffing demand $\demandj$ with a station-dependent initial range $[\pLjzero,\pRjzero]$. On each day $t\in[T]$, the platform receives a demand forecast $\prediction_t = \{[\pLjt,\pRjt]\}_{j\in[m]}$ where the interval $[\pLjt,\pRjt]$ is the prediction of demand~$\demandj$ for station $j$. As we mentioned at the beginning of this section, we assume that demand predictions are consistent (i.e., $\demandj\in[\pLjt,\pRjt]$) and have station-dependent bounded error (i.e., $\pRjt -\pLjt \leq \perrorjt$). To simultaneously fulfill all the $m$ demands $\{\demandj\}_{j\in[m]}$ on the operating day $T+1$, the platform irrevocably hires $\allocijt\in\reals_+$ available workers from pool $i$ to be assigned to station $j$ on each day $t\in[T]$, subject to the feasibility, that is,
$\sum\nolimits_{t\in[T]}\sum\nolimits_{j\in[m]}\frac{1}{\wdiscountit}\allocijt \leq \supplyi$ for every pool $i\in[n]$.
% \begin{align*}
% \begin{array}{lll}   & \forall i\in[n]:
%     &
%     \displaystyle\sum\nolimits_{t\in[T]}\sum\nolimits_{j\in[m]}\frac{1}{\wdiscountit}\allocijt \leq \supplyi
% \end{array}
% \end{align*}

\xhdr{Multi-station cost objective functions.} Given staffing profile $\xbf =\{\allocijt\}_{i\in[n],j\in[m],t\in[T]}$ and demand profile $\dbf = \{\demandj\}_{j\in[m]}$, the \emph{egalitarian-staffing cost} $\CostInf[\dbf]{\xbf}$ and \emph{utilitarian-staffing cost} $\CostOne[\dbf]{\xbf}$ are defined as:
$\CostInf[\dbf]{\xbf} \triangleq 
    \max\nolimits_{j\in[m]}
    \Cost[\demandj]{\xbf_j}$ and $
    \CostOne[\dbf]{\xbf} \triangleq 
    \sum\nolimits_{j\in[m]}\Cost[\demandj]{\xbf_j}$, respectively, 
% \begin{align*}
%     \CostInf[\dbf]{\xbf} &\triangleq 
%     \max\nolimits_{j\in[m]}
%     \Cost[\demandj]{\xbf_j},\qquad
%     \CostOne[\dbf]{\xbf} \triangleq 
%     \sum\nolimits_{j\in[m]}\Cost[\demandj]{\xbf_j}
% \end{align*}
where $\Cost[\demandj]{\xbf_j}$ is the staffing cost of station $j$ (defined in \Cref{sec:prelim}) given its staffing profile $\xbf_j= \{\allocijt\}_{i\in[n],t\in[T]}$ and demand $\demandj$.


\xhdr{The minimax optimal algorithm.}
Following the recipe in \Cref{sec:base model result}, in \Cref{sec:multi-station}, we introduce linear program~\ref{eq:opt reduced form multi station} and {\OPTSimInfty} (\Cref{alg:opt multi station}) which generalize \ref{eq:opt reduced form} and {\OPTSim} (\Cref{alg:opt}), respectively. The minimax optimality of \Cref{alg:opt multi station} follows a similar but more complicated approach as that of \Cref{thm:opt alg} and is deferred to \Cref{apx:optalginfty}. Furthermore, following the same discussion as in \Cref{sec:base model result}, it can be verified that \Cref{alg:opt multi station} is feasible and has a polynomial running time.

\begin{restatable}{theorem}{optalgmultistation}
\label{thm:opt alg multi station}
    In the multi-station environment, 
    {\OPTSimInfty} (\Cref{alg:opt multi station}) is minimax optimal. Its optimal minimax cost $\optcost$ is equal to the objective value of~\ref{eq:opt reduced form multi station}.
\end{restatable}

\vspace{-3mm}
\subsection{Workforce Planning with Costly Hiring and Discharging}
\label{sec:costly-hiring}
In this section, we consider an extension in which the platform has a budget and the hiring is costly. Moreover, in contrast to our based model, the platform is allowed to revoke previous hiring decisions after paying a cost, which we refer to as \emph{costly discharge}. 

\xhdr{The costly hiring and discharging environment.} We consider the following generalization of the base model studied in \Cref{sec:base model}. The platform has a total \emph{budget} of $\budget$ for the staffing decision. On each day~$t\in[T]$, by hiring  $\allocit\in\reals_+\cup\{\infty\}$ available workers from each pool~$i$, the platform needs to \emph{pay} $\allocit\cdot \priceit$ where $\priceit$ is the per-worker wages for pool $i$ on day $t$. Moreover, the platform can also \emph{discharge} $\revokeit\in\reals_+$ previously hired workers from each pool $i$ by paying a per-worker discharging fee $\cpriceit\in\reals_+\cup\{\infty\}$. We further assume that if a worker is hired and later discharged by the platform, she cannot be hired again for this operating day. We say a (joint hiring and discharging) staffing profile $\{\allocit, \revokeit\}_{i\in[n],t\in[T]}$ is \emph{feasible} if
it is \emph{supply feasible} ($\sum\nolimits_{t\in[T]}\frac{1}{\wdiscountit}\allocit \leq \supplyi$ for every $i\in[n]$), \emph{budget feasible} ($\sum\nolimits_{i\in[n]}\sum\nolimits_{t\in[T]}
    \priceit  \allocit + \cpriceit \revokeit\leq \budget$),
    and 
    \emph{discharging feasible} 
    ($\sum\nolimits_{t\in[k]}\revokeit \leq 
    \sum\nolimits_{t\in[k]}\allocit$ for every $i\in[n]$, $k\in[T]$).
% \begin{align*}
% \begin{array}{lrl}
% \text{(supply-feasibility)}\qquad
%     & \forall i\in[n]:
%     &\qquad
%     \displaystyle\sum\nolimits_{t\in[T]}\frac{1}{\wdiscountit}\allocit \leq \supplyi
%     \\
%     \text{(budget-feasibility)}
%     & 
%     &\qquad
%     \displaystyle\sum\nolimits_{i\in[n]}\sum\nolimits_{t\in[T]}
%     \priceit  \allocit + \cpriceit \revokeit\leq \budget
%     \\
%     \text{(discharging-feasibility)}\qquad
%     & \forall i\in[n],k\in[T]:
%     &\qquad
%     \displaystyle\sum\nolimits_{t\in[k]}\revokeit \leq 
%     \displaystyle\sum\nolimits_{t\in[k]}\allocit 
% \end{array}
% \end{align*}
% 
% Similar to \Cref{sec:multi-station}, in this subsection we make the regularity assumption about the per-worker wages (Assumption~\ref{asp:identical increasing wage}). Additionally, 
%
We also make the following structural assumption about the per-worker discharging fees.

\begin{assumption}[Piecewise stationary discharging fees]
\label{asp:limited cancellation fee}
    There exists $\cptotal\in [1:T]$ and $0 = t_0 < t_1 < t_2 < \dots < t_\cptotal = T$ such that for every index $\ell\in[\cptotal]$, the per-worker discharging fees remain identical for each time interval $[t_{\ell - 1} + 1: t_{\ell}]$, i.e., $\forall t,t'\in[t_{\ell - 1} + 1: t_{\ell}]$ and $\forall i, i'\in[n]$, we have
        $\cpriceit\equiv \cprice_{i't'}$.
\end{assumption}
% We introduce the auxiliary notation $\cintervalell\triangleq [t_{\ell - 1} + 1: t_{\ell}]$ and $\cintervalellplus \triangleq [t_{\ell - 1}: t_{\ell}]$. We refer to each of $\cintervalell$ as an \emph{epoch}. Moreover, with slight abuse of notation, we use $\cpriceiled$ to denote the per-worker discharging fee for all days $t\in\cintervalell$ in the remainder of this subsection.
% We introduce the auxiliary notation $\cintervalell\triangleq [t_{\ell - 1} + 1: t_{\ell}]$ and $\cintervalellplus \triangleq [t_{\ell - 1}: t_{\ell}]$. 
% We refer to each of $\cintervalell\triangleq [t_{\ell - 1} + 1: t_{\ell}]$ as an \emph{epoch}. 
% Moreover, with slight abuse of notation, we use $\cpriceiled$ to denote the per-worker discharging fee for all days $t\in\cintervalell$ in the remainder of this subsection.


To extend our approach to this extension, we face new challenges. First, restricting the adversary to only single-switching prediction sequences in \eqref{eq:single switch prediction construction} is not without loss. 
% As will become clear soon, 
The adversary can benefit from multiple switches to force the algorithm to hedge more through its discharging decisions. Second, it is not clear how to make discharging decisions and how to emulate them similar to Procedure~\ref{alg:emulator}.

\vspace{0mm}
\xhdr{High-level sketch of our approach.} We first introduce a larger subset of $O(T^\cptotal)$ of prediction sequences, formally described in ~\eqref{eq:multi switch prediction construction} (in contrast to $T$ prediction sequences in \eqref{eq:single switch prediction construction}). In short, since the discharging fees remain constant in each epoch $\cintervalell
% \triangleq[t_{\ell - 1} + 1: t_{\ell}]
\subseteq[T]$, we consider an adversary that follows a single-switch strategy in each epoch, such as the one introduced in \eqref{eq:single switch prediction construction} for the base model. (Note that our base model is simply a special case when when $\cptotal = 1$, $\priceit = 0$ for all $i,t$, and $\cprice_{i1} = \infty$ for all $i$.) We then concatenate these prediction sequences for different epochs $\cintervalell$ to obtain the entire prediction sequence. Using this new subset , we introduce a \emph{configuration linear program}~\ref{eq:opt cancellation} that helps us to characterize the optimal minimax cost. When $\cptotal$ is constant (which is generally satisfied in the last-mile delivery industry), program~\ref{eq:opt cancellation} has a polynomial size.

% Briefly speaking, in each constructed prediction sequence, since the discharging fees remain identical in every subinterval $\cintervalell\subseteq[T]$, our constructed predictions in $\cintervalell$ follow similar structures as the ones in \eqref{eq:single switch prediction construction} introduced for the base model.

%  Utilizing this new prediction sequence subset, we introduce a configuration linear program~\ref{eq:opt cancellation} that characterizes the optimal minimax cost. When $\cptotal$ is constant, program~\ref{eq:opt cancellation} has polynomial size.

Emulating the solution of this new program~\ref{eq:opt cancellation} for a general prediction sequence has intricacies in the extension model. We overcome them first by identifying certain properties of the minimax optimal algorithm and incorporating them directly into program~\ref{eq:opt cancellation}. Second, unlike the minimax optimal algorithms developed in previous sections that only solve an offline program once and then emulate it over the entire time horizon, the minimax optimal algorithm~\OPTSimCan\ (\Cref{alg:opt cancellation}) resolves an updated version of program~\ref{eq:opt cancellation} at the beginning of each epoch $\cintervalell$. Motivated by this resolving idea, we develop an induction argument to show the minimax optimality of \OPTSimCan. 
Note also that \OPTSimCan\ has $\texttt{Poly}(n, T^\cptotal)$ running time.
See \Cref{sec:cancellation} for details on the LP configuration and our new LP emulator algorithm. Using these components, we show the following theorem.
% Below, we explain all the details of our approach.
\vspace{0mm}
\begin{restatable}{theorem}{optalgcan}
\label{thm:opt alg cancellation}
    In the costly hiring and discharging environment and under Assumption~\ref{asp:limited cancellation fee},
    \OPTSimCan\ is minimax optimal. Its optimal minimax cost $\optcost$ is equal to the objective value of program~\ref{eq:opt cancellation}.
\end{restatable}

==> Paper/EC-macros.tex <==

\addtolength{\textheight}{1cm}
 \addtolength{\voffset}{-0.5cm}
 \addtolength{\textwidth}{0.2cm}
 \addtolength{\hoffset}{-0.1cm}

\usepackage{tikz}
\usepackage{pgfplots}
\pgfplotsset{compat=newest}
\usetikzlibrary{patterns}
\usepgfplotslibrary{fillbetween}
\usetikzlibrary{intersections}
% \usepackage{natbib}
% \setlength{\bibsep}{0.0pt}

% a very useful package for edits and comments, from David Kempe (USC)
% \usepackage{color-edits}
\usepackage[suppress]{color-edits}  % use this to suppress the package
\addauthor{yf}{purple}    % yf for Yiding
% e.g. for Yiding: \yfedit{}, \yfcomment{}, \yfmargincomment{}, \yfdelete{}.

\usepackage[caption=false]{subfig}

\usepackage{bbm}

\usepackage[breakable, skins]{tcolorbox}
\definecolor{myLightGray}{gray}{0.97} % 0 = black, 1 = white

\DeclareRobustCommand{\mybox}[2][myLightGray]{%
\begin{tcolorbox}[
        left=0.5pt,
        right=0.5pt,
        top=0.5pt,
        bottom=0.5pt,
        colback=#1,
        colframe=#1,
        width=\dimexpr\textwidth\relax, 
        boxsep=3pt,
        arc=2pt,outer arc=2pt
        ]
        #2    
\end{tcolorbox}
}
\usepackage{csquotes}
\makeatletter
%Take the original environment definition and change the leftmargin to 1cm
\renewenvironment*{displayquote}
  {\begingroup\setlength{\leftmargini}{0.25cm}\csq@getcargs{\csq@bdquote{}{}}}
  {\csq@edquote\endgroup}
\makeatother

\usepackage{mathtools, amsmath}
\usepackage{xcolor}
% \usepackage[normalem]{ulem}
\usepackage{thm-restate}
% \usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
% \usepackage[colorlinks=true, linkcolor=blue!70!black, citecolor=blue!70!black,urlcolor=blue!70!black,breaklinks=true]{hyperref}

\usepackage{comment}
% \usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{float}
\usepackage{xspace}
% \usepackage{xfrac}
\usepackage{enumitem}
\usepackage{graphicx}
% \usepackage{subfigure}
% \usepackage{subcaption}

% \usepackage{parskip}

% \usepackage{txfonts}


% Natbib setup for author-number style
\usepackage{natbib}
 \bibpunct[, ]{(}{)}{,}{a}{}{,}%
 \def\bibfont{\small}%
 \def\bibsep{\smallskipamount}%
 \def\bibhang{24pt}%
 \def\newblock{\ }%
 \def\BIBand{and}%



\usepackage{hyperref}

\usepackage{cleveref}




% \usepackage[ruled,vlined,linesnumbered]{algorithm2e} % For algorithms
\usepackage{setspace}
\usepackage{fix-cm}
\crefname{algocf}{alg.}{algs.}
\Crefname{algocf}{Algorithm}{Algorithms}
% \usepackage{algpseudocode}
% \usepackage{algorithm}
\newcommand{\algcomment}[1]{\textcolor{blue}{\footnotesize{/* \texttt{{#1}}} */}}
\newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{blue}{#1}}
\usepackage{cleveref}

\newenvironment{myprocedure}[1][htb]
{ \renewcommand{\algorithmcfname}{Procedure} %Update algorithm name
\begin{algorithm}[#1]%
}{\end{algorithm}}



\allowdisplaybreaks
\newtheorem{theorem}{Theorem}[section]
\usepackage{thm-restate}
\newtheorem{lemma}[theorem]{Lemma}
% \newtheorem*{lemma*}{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{observation}{Observation}
\newtheorem{claim}{Claim}
\newtheorem{conjecture}[theorem]{Conjecture}

\newtheorem{definition}{Definition}[section]

\newtheorem{remark}[definition]{Remark}
\newenvironment{example}[1][Example]{\begin{trivlist}
\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
% 	\newenvironment{remark}[1][Remark]{\begin{trivlist}
% \item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
	\newtheorem{assumption}[definition]{Assumption} 


	\newenvironment{numberedassumption}[1]{%
		\renewcommand{\thedefinition}{#1}%
\begin{assumption}}{\end{assumption}\addtocounter{definition}{-1}}



\newcommand{\squishlist}{
\begin{list}{{{\small{$\bullet$}}}}
{\setlength{\itemsep}{3pt}      \setlength{\parsep}{1pt}
\setlength{\topsep}{1pt}       \setlength{\partopsep}{0pt}
\setlength{\leftmargin}{1em} \setlength{\labelwidth}{1em}
\setlength{\labelsep}{0.5em} } }
\newcommand{\squishend}{  \end{list}}


\newcommand{\primed}{^{\dagger}}
\newcommand{\doubleprimed}{^{\ddagger}}

\newcommand{\xhdr}[1]{\vspace{2mm} \noindent{\bf #1}}

\newcommand{\Cost}[2][]{{\textsc{cost}}\ifthenelse{\not\equal{}{#1}}{_{#1}}{}\!\left[{\def\givenn{\middle|}#2}\right]}
\newcommand{\CostInf}[2][]{{\textsc{E-cost}}\ifthenelse{\not\equal{}{#1}}{_{#1}}{}\!\left[{\def\givenn{\middle|}#2}\right]}
\newcommand{\CostOne}[2][]{{\textsc{U-cost}}\ifthenelse{\not\equal{}{#1}}{_{#1}}{}\!\left[{\def\givenn{\middle|}#2}\right]}
\newcommand{\CostTotal}[2][]{{\widetilde{\textsc{cost}}}\ifthenelse{\not\equal{}{#1}}{_{#1}}{}\!\left[{\def\givenn{\middle|}#2}\right]}

\newcommand{\demand}{d}
\newcommand{\demandj}{\demand_j}

\newcommand{\supply}{s}
\newcommand{\supplyi}{\supply_i}

\newcommand{\wdiscount}{\rho}
\newcommand{\wdiscountDot}{\dot{\wdiscount}}
\newcommand{\wdiscountit}{\wdiscount_{it}}
\newcommand{\wdiscountDotit}{\wdiscountDot_{it}}
\newcommand{\alloc}{x}
\newcommand{\allocijt}{\alloc_{ijt}}
\newcommand{\price}{p}
\newcommand{\priceijt}{\price_{ijt}}


\newcommand{\dbf}{\boldsymbol{d}}
\newcommand{\xbf}{\boldsymbol{x}}

\newcommand{\cost}{\gamma}
\newcommand{\undercost}{c}
\newcommand{\overcost}{C}

\newcommand{\reals}{\mathbb{R}}

\newcommand{\prediction}{\mathcal{P}}
\newcommand{\predictions}{\boldsymbol{\prediction}}
\newcommand{\predictiont}{\prediction_t}
\newcommand{\pL}{L}
\newcommand{\pLjt}{\pL_{jt}}
\newcommand{\pLjzero}{\pL_{j0}}
\newcommand{\pR}{R}
\newcommand{\pRjt}{\pR_{jt}}
\newcommand{\pRjzero}{\pR_{j0}}
\newcommand{\perror}{\Delta}
\newcommand{\perrorjt}{\perror_{jt}}
\newcommand{\perrorjk}{\perror_{jk}}

\newcommand{\instance}{\mathcal{I}}

\newcommand{\ALG}{\texttt{ALG}}
\newcommand{\OPTALG}{\ALG^*}
\newcommand{\optcost}{\Gamma^*}

\newcommand{\budget}{B}

\newcommand{\undercostj}{\undercost_j}
\newcommand{\overcostj}{\overcost_j}

\newcommand{\allocit}{\alloc_{it}}
\newcommand{\priceit}{\price_{it}}
\newcommand{\pRzero}{\pR_{0}}
\newcommand{\perrork}{\perror_k}
\newcommand{\perrort}{\perror_t}
\newcommand{\OPTSimTT}{\texttt{\ref{eq:opt reduced form total cost} Emulator}}

\newcommand{\stations}{\mathcal{J}}
\newcommand{\understations}{\stations_-}
\newcommand{\overstations}{\stations_+}

\newcommand{\OPT}{\texttt{OPT}}

\newcommand{\pLzero}{\pL_0}
\newcommand{\pLt}{\pL_t}
\newcommand{\pRt}{\pR_t}
\newcommand{\pricet}{\price_t}

\newcommand{\pRtHat}{\hat{\pR}_t}
\newcommand{\pLtHat}{\hat{\pL}_t}

\newcommand{\alloct}{\alloc_t}
\newcommand{\revoke}{y}
\newcommand{\revoket}{\revoke_t}
\newcommand{\cprice}{q}
\newcommand{\cpricet}{\cprice_t}
\newcommand{\wdiscountt}{\wdiscount_t}
\newcommand{\cptotal}{L}
\newcommand{\naturals}{\mathbb{N}}
\newcommand{\elled}{^{(\ell)}}
\newcommand{\cpriceled}{\cprice_{\ell}}
\newcommand{\switchseq}{J}
\newcommand{\switchseqspace}{\mathcal{J}}
\newcommand{\switchseqell}{\switchseq_{\ell}}
\newcommand{\switchseqonetoell}{\switchseq_{1:\ell}}
\newcommand{\rgapJ}{\rgap(\switchseq)}
\newcommand{\lgapellJ}{\lgap\elled(\switchseq)}
\newcommand{\revokeellJ}{\revoke\elled(\switchseq)}
\newcommand{\revokeit}{\revoke_{it}}
\newcommand{\alloctJ}{\alloct(\switchseq)}
\newcommand{\lgapJ}{\lgap(\switchseq)}
\newcommand{\pRJ}{\pR(\switchseq,\status)}
\newcommand{\pLJ}{\pL(\switchseq,\status)}
\newcommand{\cpriceit}{\cprice_{it}}
\newcommand{\cpriceiled}{\cprice_{\ell}}
\newcommand{\cinterval}{\mathcal{T}}
\newcommand{\cintervalell}{\cinterval_{\ell}}
\newcommand{\cintervalellplus}{\cinterval_{\ell}^+}

% \newcommand{\cintervalellplusone}{\cinterval_{\ell+1}}

\newcommand{\zerobf}{\boldsymbol{0}}
\newcommand{\ybf}{\boldsymbol{y}}
\newcommand{\zbf}{\boldsymbol{z}}

\newcommand{\targetcost}{\Gamma}
\newcommand{\targetcosts}{\boldsymbol{\targetcost}}

\newcommand{\lambdabf}{\boldsymbol{\lambda}}
\newcommand{\thetabf}{\boldsymbol{\theta}}
\newcommand{\lgap}{\lambda}
\newcommand{\lgapjk}{\lgap_{jk}}
\newcommand{\lgapj}{\lgap_{j}}
\newcommand{\rgap}{\theta}
\newcommand{\rgapj}{\rgap_j}
\newcommand{\ked}{^{(k)}}
\newcommand{\halloc}{y}
\newcommand{\hallocijtk}{\halloc_{ijt}\ked}
\newcommand{\randomalloc}{X}
\newcommand{\randomallocijt}{\randomalloc_{ijt}}
\newcommand{\randomallocit}{\randomalloc_{it}}
\newcommand{\Ted}{^{(T)}}
\newcommand{\ted}{^{(t)}}

\newcommand{\canalloc}{\tilde{\alloc}}
\newcommand{\canallocit}{\canalloc_{it}}
\newcommand{\canxbf}{\tilde\xbf}

\newcommand{\csuitted}{^{\clubsuit}}
\newcommand{\spsuitted}{^{\spadesuit}}

\newcommand{\revokei}{\revoke_i}
\newcommand{\status}{S}
\newcommand{\cumalloc}{z}
\newcommand{\cumalloci}{\cumalloc_i}
\newcommand{\cumallocs}{\boldsymbol{\cumalloc}}
\newcommand{\remainsupply}{\bar{\supply}}
\newcommand{\remainsupplyi}{\remainsupply_i}
\newcommand{\remainsupplies}{\boldsymbol{\remainsupply}}
\newcommand{\remainbudget}{\bar{\budget}}

\newcommand{\initialell}{\xi}
\newcommand{\xied}{^{(\xi)}}
\newcommand{\txied}{t\xied}
\newcommand{\switchseqspaceresolve}{\switchseqspace}
\newcommand{\allocitJ}{\alloc_{it}(\switchseq)}
\newcommand{\allocizero}{\alloc_{i\txied}}
\newcommand{\revokeizero}{\revoke_i\xied}
% \newcommand{\curpL}{\pL_{t_{\ell - 1}}}
% \newcommand{\curpR}{\pR_{t_{\ell - 1}}}
\newcommand{\curpL}{\bar\pL}
\newcommand{\curpR}{\bar\pR}
\newcommand{\vtg}{\optcost}
\newcommand{\vtgstatus}{\vtg(t, \status)}
\newcommand{\supplys}{\boldsymbol{\supply}}
\newcommand{\revokeiell}{\revoke_{i\ell}}
\newcommand{\revokeiellJ}{\revoke_{i\ell}(\switchseq)}
\newcommand{\cpriceizero}{\cprice_{i0}}
\newcommand{\revokeizeroJ}{\revoke_{i0}(\switchseq)}
\newcommand{\canrevokeit}{\tilde{\revoke}_{it}}
\newcommand{\canrevokeited}{\tilde{\revoke}_{i}^{(t)}}
\newcommand{\canrevoke}{\tilde{\revoke}}

\newcommand{\randomrevoke}{Y}
\newcommand{\randomrevokeit}{\randomrevoke_{it}}
\newcommand{\cumallocBar}{\bar\cumalloc}
\newcommand{\cumallociBar}{\bar\cumalloc_i}
\newcommand{\cumallociHat}{\hat\cumalloc_i}

\newcommand{\OPTSim}{\textsc{\ref{eq:opt reduced form} Emulator}}

\newcommand{\OPTSimCan}{\textsc{\ref{eq:opt cancellation} Emulator}}

\newcommand{\OPTSimTilde}{\textsc{\ref{eq:opt variant cost} Emulator}}



	\DeclarePairedDelimiter{\abs}{\lvert}{\rvert}

\newcommand{\OPTSimInfty}{\textsc{\ref{eq:opt reduced form multi station} Emulator}}
\newcommand{\OPTSimOne}{\textsc{\ref{eq:opt reduced form multi station} Emulator}}


\newcommand{\OPTSimImperfect}{\textsc{\ref{eq:opt reduced form imperfect prediction} Emulator}}

\newcommand{\lpcancelsubproblem}{\text{\ref{eq:opt cancellation}}[\ell,\status]}

\newcommand{\RN}[1]{\textcolor{red}{\bf [Rad: #1]}}
	\newcommand{\YF}[1]{\textcolor{blue}{ (\em Yiding: \bf#1)}}
	\newcommand{\vm}[1]{\textcolor{purple}{ [V: #1]}}
 \newcommand{\VM}[1]{\textcolor{purple}{ [V: #1]}}

 \newcommand{\SN}[1]{\textcolor{orange}{\bf (Saba: #1)}}


\newcommand{\pbias}{\varepsilon}
\newcommand{\pbiass}{\boldsymbol{\predictionbias}}
\newcommand{\biaseddemand}{\hat\demand}

\newcommand{\perrors}{\boldsymbol{\perror}}
\newcommand{\predictionbias}{\pbias}
\newcommand{\predictionbiass}{\pbiass}

 \addtolength{\textheight}{0.6cm}
  \addtolength{\voffset}{-0.3cm}
  \addtolength{\textwidth}{0.2cm}
  \addtolength{\hoffset}{-0.1cm}

%  \addtolength{\textheight}{1.7cm}
% \addtolength{\voffset}{-0.85cm}
% \addtolength{\textwidth}{0.7cm}
% \addtolength{\hoffset}{-0.35cm}
%%%%%%%%%%%%%%%%



\newcommand{\dailydemand}{\delta}
\newcommand{\dailydemands}{\boldsymbol{\dailydemand}}
\newcommand{\dailydemandt}{\dailydemand_t}
\newcommand{\prior}{\xi}
\newcommand{\priors}{\boldsymbol{\prior}}
\newcommand{\priort}{\prior_t}
\newcommand{\priork}{\prior_k}

\newcommand{\dailydemandsample}{\tilde{\dailydemand}}
\newcommand{\dailydemandsamples}{\tilde{\dailydemands}}
\newcommand{\dailydemandsamplest}{\dailydemandsamples\ted}
\newcommand{\dailydemandsamplesk}{\dailydemandsamples\ked}
\newcommand{\dailydemandsampletk}{\dailydemandsample\ted_k}
\newcommand{\dailydemandsamplekt}{\dailydemandsample\ked_t}

\newcommand{\estimateddemand}{\tilde{\demand}}
\newcommand{\estimateddemandk}{\estimateddemand\ked}

==> Paper/EC-math.tex <==
\newcommand{\setsize}[1]{{\left|#1\right|}}





\newcommand{\super}[1]{^{(#1)}}

\newcommand{\interval}[1]{\Big[#1\Big]}
\newcommand{\tinteval}[1]{\left[#1\right]}
\newcommand{\distcond}[2]{\left.#1\vphantom{\big|}\right|_{#2}}
\newcommand{\evalat}[2]{\left.#1\vphantom{\big|}\right|_{#2}}


%
% probability stuff.
%
\newcommand{\condition}{\,\mid\,}

% resizing brackets 
\newcommand{\prob}[2][]{\text{Pr}\ifthenelse{\not\equal{}{#1}}{_{#1}}{}\!\left[{\def\givenn{\middle|}#2}\right]}
\newcommand{\expect}[2][]{\mathbb{E}\ifthenelse{\not\equal{}{#1}}{_{#1}}{}\!\left[{\def\givenn{\middle|}#2}\right]}


\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

% brackets configured with \tparen
\newcommand{\tparen}{\big}
\newcommand{\tprob}[2][]{\text{Pr}\ifthenelse{\not\equal{}{#1}}{_{#1}}{}\tparen[{\def\given{\tparen|}#2}\tparen]}
\newcommand{\texpect}[2][]{\mathbb{E}\ifthenelse{\not\equal{}{#1}}{_{#1}}{}\tparen[{\def\given{\tparen|}#2}\tparen]}


% brackets do not resize.
\newcommand{\sprob}[2][]{\text{Pr}\ifthenelse{\not\equal{}{#1}}{_{#1}}{}[#2]}
\newcommand{\sexpect}[2][]{\mathbb{E}\ifthenelse{\not\equal{}{#1}}{_{#1}}{}[#2]}






\newcommand{\suchthat}{\,:\,}


\newcommand{\partialx}[2][]{{\tfrac{\partial #1}{\partial #2}}}
\newcommand{\nicepartialx}[2][]{{\nicefrac{\partial #1}{\partial #2}}}
\newcommand{\dd}{{\mathrm d}}
\newcommand{\ddx}[2][]{{\tfrac{\dd #1}{\dd #2}}}
\newcommand{\niceddx}[2][]{{\nicefrac{\dd #1}{\dd #2}}}
\newcommand{\grad}{\nabla}

\newcommand{\symdiff}{\triangle}



\newcommand{\indicator}[1]{{\mathbbm{1}\left\{ #1 \right\}}}

\newcommand{\plus}[1]{{\left( #1 \right)^+}}





==> Paper/apx-extension.tex <==
\label{apx-multi}
In this appendix section, we provide full details of the missing parts in \Cref{sec:extension}, and fill all the gaps in our technical argument in that section.

% \subsection{Minimax Optimal Algorithm for Multi-stations with Utilitarian-staffing Cost.}
% \label{sec:util}
% % \vm{if you agree with bringing this forward, please comment the sentence and the assumption.}
% % For utilitarian-staffing cost, we make the following natural regularity assumption about the per-worker wages.
% % \begin{assumption}
% % \label{asp:identical increasing wage}
% %     For every pool $i\in[n]$, its per-worker wages $\{\priceit\}_{t\in[T]}$ weakly increases in $t\in[T]$.
% % \end{assumption}
% Similar to our technical development before in \Cref{sec:ega}, consider the following modified linear program with variables $\{\allocijt,\lgapj,\rgapj\}_{i\in[n],j\in[m],t\in[T]}$ that is going to characterize the optimal minimax cost:
% \begin{align}
% \tag{$\textsc{LP-Multi-util}$}
%     \label{eq:opt reduced form L one}
%     &\arraycolsep=1.4pt\def\arraystretch{2.2}
%     \begin{array}{llll}
%     \min\limits_{\substack{\xbf,\lambdabf,\thetabf\geq \zerobf}}
%     \qquad
%     &
%     \displaystyle\sum\nolimits_{j\in[m]}
%     \undercost\cdot \rgapj
%     & 
%     \text{s.t.}
%     \\
%     &
%     \displaystyle\sum\nolimits_{t\in[T]}\frac{1}{\wdiscountit}\cdot\sum\nolimits_{j\in[m]}\allocijt \leq \supplyi
%     &
%     i\in[n]
%     \\
%     &
%     \displaystyle\sum\nolimits_{i\in[n]}\sum\nolimits_{j\in[m]}
%     % \left(
%     \sum\nolimits_{t\in[T]}
%     \priceit \cdot \allocijt 
%     % +
%     % \sum\nolimits_{t\in[k+1:T]}
%     % \priceit \cdot \hallocijtk
%     % \right)
%     \leq \budget
%     \quad
%     &
%     % k\in[0:T]
%     \\
%     &
%     \displaystyle\sum\nolimits_{i\in[n]}\sum\nolimits_{t\in[k]}
%     \allocijt \leq \pRjzero - \perrorjk + \lgapj
%     \quad
%     &
%     j\in[m], k\in[T]
%     \\
%     &
%     \displaystyle\sum\nolimits_{i\in[n]}\sum\nolimits_{t\in[T]}
%     \allocijt \geq \pRjzero - \rgapj
%     &
%     j\in[m]
%     \\
%     &\overcost \cdot \lgapj \leq \undercost\cdot \rgapj & j\in[m]
% \end{array}
% \end{align}
% Compared to programs~\ref{eq:opt reduced form} for the base model and~\ref{eq:opt reduced form L infty} for the egalitarian-staffing cost, this new program introduces a new constraint that $\overcost \cdot \lgapj \leq \undercost\cdot \rgapj$ for all station $j$. This additional constraint turns out to be the key in the analysis showing that the staffing cost of \OPTSimOne\ (defined below) is at most the objective value of program~\ref{eq:opt reduced form L one} for all prediction sequences. 

% Now we present the minimax optimal algorithm for utilitarian-staffing cost (\Cref{alg:opt L one}) with its guarantee of optimality (\Cref{thm:opt alg L one}). Similarly to \Cref{alg:opt L infty}, this new algorithm can be directly shown to be budget- and supply-feasible and has a polynomial running time.

% \begin{algorithm}
%     \SetKwInOut{Input}{input}
%     \SetKwInOut{Output}{output}
%     \Input{prediction sequence $\predictions=\{[\pLjt,\pRjt]\}_{j\in[m],t\in[T]}$ revealed sequentially over time}
%     \Output{staffing profile $\xbf$}
%     \vspace{2mm}
%     find an optimal solution $(\xbf^*, \lambdabf^*, \thetabf^*)$ of program~\ref{eq:opt reduced form L one}
    
%     \vspace{2mm}
%     \For{each station $j\in[m]$}{
%     invoke Procedure~\ref{alg:emulator} with canonical staffing profile $\canxbf \gets \{\allocijt^*\}_{i\in[n],t\in[T]}$ and prediction sequence $\tilde\predictions\gets \{[\pLjt,\pRjt]\}_{t\in[T]}$ for station $j$
%     }
%     \caption{\OPTSimOne}
%     \label{alg:opt L one}
% \end{algorithm}

% \optalgone*


% The proof of \Cref{thm:opt alg L one} also follows a similar approach to the proof of \Cref{thm:opt alg}.
% As mentioned above, the main difference is that the new constraint $\overcost \cdot \lgapj \leq \undercost\cdot \rgapj$ in program~\ref{eq:opt reduced form L one} enables us to compare the cost guarantee of \OPTSimOne\ with the optimal objective value of program~\ref{eq:opt reduced form L one} (\Cref{lem:opt alg minimax cost L one}). However, due to this additional constraint, showing that program~\ref{eq:opt reduced form L one} lower bounds the optimal minimax cost becomes more challenging. We overcome this challenge by first introducing a modified program~\ref{eq:opt reduced form L one modified}, showing it lower bounds the optimal minimax cost, and finally arguing that the optimal solution in program~\ref{eq:opt reduced form L one modified} can be converted into a feasible solution for program~\ref{eq:opt reduced form L one} under \Cref{asp:identical increasing wage} (\Cref{lem:opt reduced form lower bound optimal minimax cost L one,lem:opt reduced form lower bound optimal minimax cost L one modified,lem:L infty overcost vs undercost}). See the formal analysis in \Cref{apx:optalgone}.




\subsection{More Details on Minimax Optimal Algorithm with Costly Discharge}
\label{apx:discharge}
In the following, we elaborate on the remaining technical parts of \Cref{sec:cancellation}, and prove the main result of that section, that is, an LP-based emulator algorithm for the costly discharging environment.

We introduce the auxiliary notation $\cintervalell\triangleq [t_{\ell - 1} + 1: t_{\ell}]$ and $\cintervalellplus \triangleq [t_{\ell - 1}: t_{\ell}]$. We refer to each of $\cintervalell$ as an \emph{epoch}. Moreover, with slight abuse of notation, we use $\cpriceiled$ to denote the per-worker discharging fee for all days $t\in\cintervalell$ in the remainder of this subsection.

\xhdr{Configuration LP for the optimal minimax cost.} We describe the subset of prediction sequences  that inspires linear program~\ref{eq:opt cancellation}. First, we introduce the auxiliary notation -- \emph{configuration $\switchseq\in{\times}_{\ell\in[\cptotal]}\cintervalellplus$} and denote $\switchseqspace\triangleq{\times}_{\ell\in[\cptotal]}\cintervalellplus$ as the space of all configurations. As a sanity check, $|\switchseqspace| = O(T^\cptotal)$. Moreover, for any configuration $\switchseq$, we use $\switchseqell \in \cintervalellplus$ to denote its $\ell$-th element, and $\switchseqonetoell \in {\times}_{\ell'\in[\ell]}\cinterval_{\ell'}^+$ to denote its length-$\ell$ prefix. 

Intuitively speaking, configuration $\switchseq\in\switchseqspace$ encodes a prediction sequence $\predictions(\switchseq)= \{[\pL_t(\switchseq),\pR_t(\switchseq)]\}_{t\in[T]}$ constructed as follows:
\begin{align}
\label{eq:multi switch prediction construction}
\begin{array}{lll}
    \ell\in[\cptotal], t\in[t_{\ell - 1} + 1, \switchseqell]:&
    \qquad
    \pLt(\switchseq) \gets \pR_{t - 1}(\switchseq) - \perrort,\quad &
    \pRt(\switchseq) \gets \pR_{t - 1}(\switchseq);
    \\
    \ell\in[\cptotal], t\in[\switchseqell + 1: t_{\ell}]:&
    \qquad
    \pLt(\switchseq) \gets \pL_{t - 1}(\switchseq),\quad &
    \pRt(\switchseq) \gets \pL_{t - 1}(\switchseq) + \perrort.
\end{array}
\end{align}
where $\pLzero(\switchseq) = \pLzero$ and $\pRzero(\switchseq) = \pRzero$. The idea of using this subset is highly non-trivial and substantially reduces the dimensionality of the adversary's problem.\footnote{We note that the constructed subset of prediction sequences $\{\predictions(\switchseq)\}_{\switchseq\in\switchseqspace}$ has $O(T^\cptotal)$ prediction sequences, while the the original prediction sequence space is infinite and uncountable.} To see why, note that construction~\eqref{eq:multi switch prediction construction} ensures that for any two configurations $\switchseq,\switchseq'\in\switchseqspace$, if $\switchseq$ has the same length-$(\ell-1)$ prefix as $\switchseq'$, i.e., $\switchseq_{1:\ell-1} = \switchseq_{1:\ell-1}'$, then predictions $[\pLt(\switchseq),\pRt(\switchseq)]$ and $[\pLt(\switchseq'),\pRt(\switchseq')]$ are identical for every day $t\in[\switchseq_{\ell}\wedge\switchseq_{\ell}']$. Therefore, if we use $\allocitJ$ to denote the number of workers hired from pool $i$ on day $t$ given the prediction sequence $\predictions(\switchseq)$, the following equality should hold for any online algorithm:
\begin{align}
\label{eq:identical allocation constraint}
    \forall\ell\in[\cptotal],
    \forall\switchseq,\switchseq'\in\switchseqspace,
    \switchseq_{1:\ell-1} = \switchseq'_{1:\ell-1},
    \forall t\in[\switchseq_{\ell}\wedge\switchseq_{\ell}']:
    \qquad
    \allocitJ = \allocit(\switchseq')
\end{align}
Similarly, if we use $\revokeiellJ$ to denote the number of workers discharged from pool $i$ during days in $\cintervalell$ given prediction sequence $\predictions(\switchseq)$, the following equality should hold for any online algorithm:\footnote{Since  the per-worker discharging fee remains the same for all days in each $\cintervalell$, it is without loss of generality to assume that online algorithms only discharge workers on days $t_1, t_2, \dots, t_L$. Thus, it suffices to introduce a single variable to denote the discharging during days in $\cintervalell$ for each pool.}
\begin{align}
\label{eq:identical cancellation constraint}
    \forall\ell\in[\cptotal],
    \forall\switchseq,\switchseq'\in\switchseqspace,
    \switchseq_{1:\ell} = \switchseq'_{1:\ell}:
    \qquad
    \revokeiellJ = \revokeiell(\switchseq')
\end{align}
Due to the technical reason which we will explain later, from now on we assume that is $\cumalloci$ workers hired from pool $i$ on day 0.\footnote{Both our base and multi-station model then corresponds to $\cumalloci = 0$.}
% and consequently the platform can make an additional cancellation decision $\revokeizeroJ$ on day 0 with per-worker cancellation fee $\cpriceizero$ for pool $i$. 
The feasibility of the staffing profile can be expressed as 
\begin{align}
\label{eq:all feasibility constraint}
    \begin{split}
    \forall i\in[n],
    \forall\switchseq\in\switchseqspace:&
    \qquad
    \displaystyle\sum\nolimits_{t\in[T]}\frac{1}{\wdiscountit} \allocitJ 
    \leq 
    \supplyi
    \\
    \forall \switchseq\in\switchseqspace:&
    \qquad
    \displaystyle\sum\nolimits_{i\in[n]}
    \left(
    \sum\nolimits_{t\in[T]}
    \priceit\allocitJ
    +
    \sum\nolimits_{\ell\in[\cptotal]}
    \cpriceiled\revokeiellJ
    \right)
    \leq \budget
    \\
    \forall i\in[n],
    \forall\ell\in[\cptotal],
    \forall\switchseq\in\switchseqspace:&
    \qquad
    \displaystyle
    \sum\nolimits_{\ell'\in[\ell]}\revoke_{i\ell'}(\switchseq)
    \leq
    \cumalloci + 
    \sum\nolimits_{t\in[t_\ell]}\allocitJ 
    \end{split}
\end{align}
Suppose we use $\lgapJ$ and $\rgapJ$ to denote the largest possible overstaffing and understaffing given prediction sequence $\predictions(\switchseq)$, we have
\begin{align}
\label{eq:bounded cost constraint}
\begin{split}
    \forall \switchseq\in\switchseqspace:&
    \qquad
    \sum\nolimits_{i\in[n]}
    \left(
    \cumalloci + \sum\nolimits_{t\in[T]}\allocitJ
    -
    \sum\nolimits_{\ell\in[\cptotal]}\revokeiellJ
    \right)
    \leq
    \pL_T(\switchseq) + \lgapJ
    \\
% \label{eq:undercost constraint}
    \forall \switchseq\in\switchseqspace:&
    \qquad
    \sum\nolimits_{i\in[n]}
    \left(
    \cumalloci + \sum\nolimits_{t\in[T]}\allocitJ
    -
    \sum\nolimits_{\ell\in[\cptotal]}\revokeiellJ
    \right)
    \geq
    \pR_T(\switchseq) - \rgapJ
\end{split}
\end{align}
% Finally, we impose the following two structural constraints over the staffing profiles. Our analysis shows that both of them are satisfied by the minimax optimal algorithm.
% \begin{align}
% % \label{eq:no allocation after switch constraint}
% %     \forall \ell\in[\cptotal],
% %     \forall \switchseq\in\switchseqspace,
% %     \forall t\in[\switchseqell + 1: t_{\ell}],\forall i\in[n]:&
% %     \qquad 
% %     \allocitJ = 0 
% %     \\
% \label{eq:prefer early allocation constraint}
%     \forall \ell\in[\cptotal],
%     \forall \switchseq\in\switchseqspace,
%     % \switchseqell = t_\ell,
%     t\in\cintervalell,t\geq 2:&
%     \qquad
%     \sum\nolimits_{i\in[n]}\allocitJ \leq \pL_{t}(\switchseq) - \pL_{t-1}(\switchseq)
% \end{align}
% and
% \begin{align}
% \label{eq:early switch higher cumalloc constraint}
% \begin{split}  
% \forall \ell\in[\cptotal],
% \forall\switchseq,\switchseq'\in\switchseqspace,
% \switchseq_{1:\ell-1} = \switchseq_{1:\ell-1}',
% \switchseq_{\ell} < \switchseq_{\ell}':
% \qquad
% \qquad
% \qquad
% \qquad
% \qquad
% \qquad
% \qquad
% \qquad
% \\
%     \sum\nolimits_{i\in[n]}
% \left(
% \sum\nolimits_{t\in\cinterval_{\ell}}\left(\allocitJ
% -
% \allocit(\switchseq')
% \right)
% -
% \left(
% \revokeiellJ
% -
% \revokeiell(\switchseq')
% \right)
% \right)
% -
% \left(
% \pL_{t_{\ell}}(\switchseq)
% -
% \pL_{t_{\ell}}(\switchseq')
% \right)
% \geq 0
% \end{split}
% \end{align}
% Here constraint~\eqref{eq:prefer early allocation constraint} follows a similar intuition behind the construction of \Cref{alg:opt simple instance} given \Cref{asp:identical increasing wage}. Constraint~\eqref{eq:early switch higher cumalloc constraint} is implied by the intuition as follows: consider two prediction sequence $\predictions(\switchseq)$ and $\predictions(\switchseq')$ where all predictions before subinterval $\cintervalell$ are the same. Suppose at the end of day $t_\ell$, the overstaffing before applying cancellation $\revokeiellJ$ is weakly higher in  $\predictions(\switchseq)$ than $\predictions(\switchseq')$. Then the overstaffing after applying cancellation $\revokeiellJ$ is also weakly higher in $\predictions(\switchseq)$ than $\predictions(\switchseq')$.

We now present linear program~\ref{eq:opt cancellation} that characterizes the optimal minimax cost:
\begin{align}
\tag{$\textsc{LP-discharge}$}
    \label{eq:opt cancellation}
    % &\arraycolsep=1.4pt\def\arraystretch{2.2}
    \begin{array}{llll}
    \min\limits_{\substack{\xbf,\ybf,\lambdabf,\thetabf\geq \zerobf}}
    &
    \max\limits_{\switchseq\in\switchseqspace}
    \undercost\cdot\rgapJ
    \vee
    \overcost\cdot\lgapJ
    \quad
    & 
    \text{s.t.}
    \\
    &
    \text{constraints}~\labelcref{eq:identical allocation constraint,eq:identical cancellation constraint,eq:all feasibility constraint,eq:bounded cost constraint} 
\end{array}
\end{align}



As we discussed earlier, the optimal minimax algorithm for the costly discharging environment repeatedly resolves program~\ref{eq:opt cancellation} at the beginning of each day $t_\ell$, $\ell\in[\cptotal]$ by viewing the staffing decisions in the remaining time horizon $[t_\ell: T]$ as a new subproblem. We use $\status$ to denote the \emph{initial state} of this subproblem. Here $\status \triangleq (\ell, \bar\cumallocs,\remainsupplies,\remainbudget,[\curpL,\curpR])$ is a tuple where $\cumallocs=\{\bar\cumalloci\}_{i\in[n]}$ is the total number of workers hired before the end of day $t_{\ell-1}$ from each pool $i$, $\remainsupplies=\{\remainsupplyi\}_{i\in[n]}$ is the number of available workers remaining in each pool $i$ at the end of day $t_{\ell - 1}$, $\remainbudget$ is the remaining budget at the end of day $t_{\ell - 1}$, and $[\curpL,\curpR]$ is the prediction revealed on day $t_{\ell - 1}$. See the formal definitions in \eqref{eq:status update}. We use $\lpcancelsubproblem$ to denote the \emph{subprogram} solved at the beginning of day $t_{\ell}$ given initial state $\status$. Specifically, the primitives in program~\ref{eq:opt cancellation} are assigned as 
\begin{align*}
    \cumallocs \gets \bar\cumallocs, ~~
    \supplys\gets\remainsupplies, ~~
    \budget\gets \remainbudget,~~
    \pLzero\gets \curpL,~~\pRzero\gets \curpR,~~
    \{\wdiscountit\}_{t\in[t_{\ell - 1} + 1:T]} \gets 
    \{\tfrac{\wdiscountit}{\wdiscount_{it_{\ell-1}}}\}_{t\in[t_{\ell - 1} + 1:T]}
\end{align*}
and all index sets (e.g., $[T], [\cptotal]$), configuration space $\switchseqspace$ are adjusted correspondingly.

\xhdr{The minimax optimal algorithm and analysis.} 
Now we present the minimax optimal algorithm --- \OPTSimCan (\Cref{alg:opt cancellation}) with its feasibility (\Cref{lem:alg feasibility cancellation}) and optimality guarantee (\Cref{thm:opt alg cancellation}). 

In \OPTSimCan, there are $\cptotal$ phases, corresponding to subintervals/epochs $\cintervalell$ for each $\ell\in[\cptotal]$. Specifically, at the end of day $t_{\ell - 1}$, given the current staffing profile $\{\allocit,\revokeit\}_{i\in[n],t\in[t_{\ell - 1}]}$ and prediction $[\pL_{t_{\ell-1}},\pR_{t_{\ell-1}}]$, the algorithm updates the initial state $\status$ as follows:
\begin{align}
\begin{split}
\label{eq:status update}
    \forall i\in[n]:&\qquad 
    \cumalloci \gets \sum\nolimits_{t\in[t_{\ell - 1}]}\allocit - \revokeit,\quad
    \remainsupplyi \gets \wdiscount_{it_{\ell - 1}}\left(\supplyi - \sum\nolimits_{t\in[t_{\ell - 1}]}\frac{1}{\wdiscountit}\allocit\right),
    \\
    &\qquad 
    \remainbudget \gets \budget - \sum\nolimits_{i\in[n]}\sum\nolimits_{t\in[t_{\ell - 1}]}\priceit\allocit+\cpriceit\revokeit,\quad
    \curpL \gets \pR_{t_{\ell - 1}} - \perror_{t_{\ell - 1}},\quad
    \curpR \gets \pR_{t_{\ell - 1}}.
\end{split}
\end{align}
The algorithm solves subprogram $\lpcancelsubproblem$ given the updated initial state $\status$ and obtains its optimal solution $\{\allocitJ^*,\revoke_{i\ell'}^*(\switchseq),\lgapJ^*,\rgapJ^*\}_{i\in[n],t\in[t_{\ell- 1} + 1:T],\ell'\in[\ell:L],\switchseq\in\switchseqspace_{\ell:L}}$ where $\switchseqspace_{\ell:L}$ is defined as $\switchseqspace_{\ell:L}\triangleq \times_{\ell'\in[\ell:L]}\cinterval_{\ell'}^+$.
The algorithm then constructs the canonical hiring decision $\{\canallocit\}_{i\in[n],t\in\cintervalell}$ as follows:
\begin{align}
\label{eq:canalloc construction}
    \forall i\in[n],\forall t\in\cintervalell:\qquad
    \canallocit \gets \allocit^*(\switchseq^{(t_{\ell})})
\end{align}
where $\switchseq^{(t_{\ell})}$ is an arbitrary sequence such that $\switchseq^{(t_{\ell})}_1 = t_{\ell}$.\footnote{For any configuration $\switchseq\in\switchseqspace_{\ell:L}$, recall $\switchseq_1$ specifies a day in $\cintervalellplus$. Due to constraint~\eqref{eq:identical allocation constraint}, all configurations $\switchseq$ such that $\switchseq_1 = t_{\ell}$ have the same $\allocitJ$ for $t \in[\cintervalell]$.}
Similarly, the algorithm constructs the canonical discharging decision $\{\canrevokeited\}_{i\in[n],t\in\cintervalellplus}$ as follows:
\begin{align*}
% \label{eq:cancellation construction}
    \forall i\in[n],\forall t\in\cintervalellplus:\qquad
    \canrevokeited \gets \revokeiell^*(\switchseq^{(t)})
\end{align*}
where $\switchseq^{(t)}$ is an arbitrary sequence such that $\switchseq^{(t)}_1 = t$.\footnote{Due to constraint~\eqref{eq:identical cancellation constraint}, all configurations $\switchseq$ such that $\switchseq_1 = t$ have the same $\revokeiellJ$.}
Similar to all minimax optimal algorithms in previous models, \OPTSimCan\ implements Procedure~\ref{alg:emulator} with canonical hiring decision $\{\canallocit\}_{i\in[n],t\in\cintervalell}$ constructed above as its input to determine the actual hiring decisions for every day $t\in\cintervalell$. Additionally, on day $t_{\ell}$, the algorithm identifies the largest index $k\in\cintervalellplus$ satisfying\footnote{Such index $k$ always exists, since this equality holds trivially for $k = t_{\ell - 1}.$}
\begin{align}
\label{eq:critical day cancellation}
    \pR_{k} - \sum\nolimits_{i\in[n]}\sum\nolimits_{t\in[t_{\ell - 1}+1:k]}\allocit =
    \pR_{t_{\ell-1}} - \sum\nolimits_{i\in[n]}\sum\nolimits_{t\in[t_{\ell - 1}+1:k]}\canallocit
\end{align}
The algorithm then uses canonical discharging decision $\{\canrevoke_i\ked\}_{i\in[n]}$ to determine the actual discharging decision $\{\revoke_i\}_{i\in[n]}$, i.e., $\revoke_i$ hired workers are discharged from pool $i$ on day $t_{\ell}$. Specifically, it computes $\{\revoke_i\}_{i\in[n]}$ as an arbitrary solution such that
\begin{align}
    \label{eq:actual cancellation construction}
    \begin{split}
    \forall i\in[n]:&\qquad 0\leq \revoke_i \leq \canrevoke_{ik}
    \\
    &\qquad 
    \sum\nolimits_{i\in[n]}
\left(
\sum\nolimits_{t\in[t_{\ell-1} +1:k]}\left(
\canallocit
-
\allocit
\right)
-
\left(
\canrevoke_{i}\ked
-
\revoke_i
\right)
\right)
=
\pR_{t_{\ell}}(\switchseq\ked)
-
\pR_{t_{\ell}}
    \end{split}
\end{align}
where $\pR_{t_{\ell}}(\switchseq\ked) = \pR_{t_{\ell - 1}} - \perror_k + \perror_{t_\ell}$ by construction~\eqref{eq:multi switch prediction construction}.
If no feasible solution satisfies condition~\eqref{eq:actual cancellation construction}, the algorithm makes no discharging on day $t_{\ell}$.

Finally, if $\ell < [\cptotal]$, the algorithm moves from phase $\ell$ to phase $\ell + 1$ and repeats.
\begin{algorithm}
    \SetKwInOut{Input}{input}
    \SetKwInOut{Output}{output}
    \Input{prediction sequence $\predictions=\{[\pLt,\pRt]\}_{t\in[T]}$ revealed sequentially over time}
    \Output{staffing profile $(\xbf,\ybf)$}
    \vspace{2mm}
    
    \For{each $\ell\in[\cptotal]$}{
    
    \vspace{1mm}

    update initial state $\status$ using \eqref{eq:status update} at the end of day $t_{\ell-1}$

    \vspace{2mm}
    
    find an optimal solution $(\xbf^*, \ybf^*, \lambdabf^*, \thetabf^*)$ of subprogram~$\lpcancelsubproblem$

    \vspace{2mm}

    invoke Procedure~\ref{alg:emulator} with canonical staffing profile $\canxbf$ constructed in \eqref{eq:canalloc construction} and prediction sequence $\predictions$ for each day $t \in \cintervalell$

    \vspace{2mm}

    \If{there exists discharging decision $\{\revoke_i\}_{i\in[n]}$ satisfying condition \eqref{eq:actual cancellation construction}}{
    
    \vspace{1mm}

    discharge $\revoke_i$ hired workers from each pool $i$ on day $t_{\ell}$
    }
    }
    
    \caption{\OPTSimCan}
    \label{alg:opt cancellation}
\end{algorithm}

\begin{remark}
    \OPTSimCan\ has $\texttt{Poly}(n, T^\cptotal)$ running time.
\end{remark}

\begin{remark}
    \OPTSimCan\ recovers \OPTSim\ when $\cptotal = 1$ and $\cprice_{i1} = \infty$ for all $i$.
\end{remark}

\begin{restatable}{lemma}{optalgcanfeasibility}
\label{lem:alg feasibility cancellation}
    In the costly discharging environment,
    the staffing profile outputted by \OPTSimCan\ is feasible.
\end{restatable}
The proof of \Cref{lem:alg feasibility cancellation} (see \Cref{apx:optalgcanfeasibility}) utilizes the properties of Procedure~\ref{alg:emulator} established in \Cref{lem:emulator} and the structural properties about the implementation of discharging decisions in \eqref{eq:actual cancellation construction}.

\optalgcan*

The proof of \Cref{thm:opt alg cancellation} (see \Cref{apx:optalgcan}) follows a similar high-level idea as the proofs of \Cref{thm:opt alg,thm:opt alg L infty,thm:opt alg L one}. We first argue that program~\ref{eq:opt cancellation} upper bounds the optimal minimax cost. We then use an induction argument (backward over index $\ell$) showing that the optimal objective of subprogram~$\lpcancelsubproblem$ is at most the cost guarantee of \OPTSimCan\ from phase $\ell$ to phase $\cptotal$ given initial state $\status$.







==> Paper/discussion.tex <==
\label{sec:discussion}
\rncomment{discussion section to talk about practical relevance of our model in the appendix, to make things more explicit; to be written}\rncomment{let's not add this?}
